Loop space of a K\"ahler manifold

We prove that the loop space of a K\"ahler manifold inherits a K\"ahler structure. Then we prove that equipped with this natural metric the loop space is complete and unbounded. Additionally, we show that a geodesic on the loop space can be constructed by piecing together geodesics from each individual leaf.

==> comments.tex <==
\ProvidesFile{Ucyril.fd}[WNCyr Font]
\DeclareFontFamily{U}{wncyr}{}
\DeclareFontShape{U}{wncyr}{m}{n}{<-6>wncyr5<6-8>wncyr7<8->wncyr10}{}
\ProcessOptions

\font\cyr  wncyr10 at 12pt
\font\cyrsm  wncyr10 at 9pt
%\font\cyrb wncyb10 at 12pt

%% wncyr special characters:
%% http://home.vrweb.de/~was/x/pmcyr.pdf
%% E0 and e0   for "e (yo (-mayo))
%% i0 and I0   for j 
%% i1 and I1   for ukr/starorussk. i s tochkoj 
%% N0          for No ("nomer")
%% Kh/kh ili H/h  for "x"  ("xiter")
%% Ts/ts ili C/c  for "tse"
%% Ch/ch ili Q/q  for "che"
%% X/x ili Sh/sh   for "sha"
%% W/w ili shch   for "scha"
%% Ya/ya ili J1/j1  for "ya"
%% Yu/yu ili J2/j2  for "yu"       


%% Vkliuchit' rus : \cyr ili \cyrb ili \cyrsm (cyrillic-small)
%% Nazad : \rm ili \bf ili \sl itd.


%% Remarki na polyax
%for margin notes
{\catcode`\@=11
\gdef\n@te#1#2{\leavevmode\vadjust{%
 {\setbox\z@\hbox to\z@{\strut#1}%
  \setbox\z@\hbox{\raise\dp\strutbox\box\z@}\ht\z@=\z@\dp\z@=\z@%
  #2\box\z@}}}
\gdef\leftnote#1{\n@te{\hss#1\quad}{}}
\gdef\rightnote#1{\n@te{\;\kern-\leftskip#1\hss}{\moveright\hsize}}
\gdef\?{\FN@\qumark}
\gdef\qumark{\ifx\next"\DN@"##1"{\leftnote{\rm##1}}\else
 \DN@{\leftnote{\rm??}}\fi{\rm??}\next@}}
%
\def\lnote#1{\leftnote{\vbox{\hsize=2truecm
\baselineskip =11pt \lineskiplimit =1pt
\footnotesize \noindent #1}}}
%
\def\rnote#1{\rightnote{\vbox{\hsize=1.5truecm
\lineskip =11pt \lineskiplimit =1pt
\tiny \noindent #1}}}
%
%
%% Kommandy : \lnote{Text} ili \rnote{Text}
%% Ili \lnote{\cyr Text} 
%%
%%


%% Cveta:
%% Available colors:
%% \red, \green, \black, \blue \magent

\usepackage[usenames,dvips]{color}

\definecolor{DarkGreen}{rgb}{0,0.6,0} 
\def\red{\color{red}}
\def\green{\color{DarkGreen}}
\def\blue{\color{blue}}
\def\black{\color{black}}
\definecolor{MyMagenta}{rgb}{0.6,0.0,0.5} 
\def\magent{\color{MyMagenta}}

%\endinput
